Connectivity augmentation is fixed-parameter tractable

In the vertex connectivity augmentation problem, we are given an undirected $n$-vertex graph $G$, a set of links $L \subseteq \binom{V(G)}{2} \setminus E(G)$, and integers $\lambda$ and $k$. The task is to insert at most $k$ links from $L$ to $G$ to make $G$ $\lambda$-vertex-connected. We show that the problem is fixed-parameter tractable (FPT) when parameterized by $\lambda$ and $k$, by giving an algorithm with running time $2^{O(k \log (k + \lambda))} n^{O(1)}$. This improves upon a recent result of Carmesin and Ramanujan [SODA'26], who showed that the problem is FPT parameterized by $k$ but only when $\lambda \le 4$. We also consider the analogous edge connectivity augmentation problem, where the goal is to make $G$ $\lambda$-edge-connected. We show that the problem is FPT when parameterized by $k$ only, by giving an algorithm with running time $2^{O(k \log k)} n^{O(1)}$. Previously, such results were known only under additional assumptions on the edge connectivity of $G$.

==> Preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}
\pdfoutput=1

\usepackage{microtype}
\usepackage{mdframed}
\usepackage{csquotes}
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}
\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amssymb}
\usepackage{amstext}
\usepackage{graphicx,tikz-cd}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage{todonotes}
\usepackage{textpos}
%%%%%
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{makecell}
\usepackage{thmtools, thm-restate}
\usepackage{thm-autoref}
 \usepackage{mathdots}
%\usepackage{wrapfig}
\usepackage{multirow}
%\usetikzlibrary{cd}
\usepackage{chngcntr}
\usepackage{apptools}
\usepackage{accents}
\usepackage{lineno}
%\linenumbers
\AtAppendix{\counterwithin{lemma}{section}}

  


\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\numberwithin{equation}{section}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{hypothesis}[equation]{Hypothesis}
\newtheorem{claim}[equation]{Claim}
\newtheorem{definition}[equation]{Definition}
\newtheorem{observation}[equation]{Observation}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{mainlemma}[equation]{Main lemma}
%\newtheorem{redrule}[lemma]{Reduction Rule}
%\newtheorem{remark}[lemma]{Remark}
%\newtheorem{reduction}[lemma]{Reduction Rule}
%\newtheorem{conjecture}[lemma]{Conjecture}
\newcommand{\cqed}{\ensuremath{\lhd}}
\makeatletter
\newenvironment{claimproof}{\par
  \pushQED{\cqed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item\relax
  {\itshape
    Proof of the claim\@addpunct{.}}\hspace\labelsep\ignorespaces
}{%
  \hfill\popQED\endtrivlist\@endpefalse
}
\makeatother


\date{}


\usepackage{booktabs}

\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hypertexnames = false,
                 hyperfigures
                 ]{hyperref}

\usepackage[nameinlink]{cleveref}
\crefname{observation}{Observation}{Observations}
\crefname{claim}{Claim}{Claims}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\crefname{mainlemma}{Main lemma}{Main lemmas}




\newcommand{\OO}{\mathcal{O}}
\DeclareMathOperator{\polylog}{polylog}

%Define in defs
\newcommand{\primal}{\mathcal{P}}
\newcommand{\bd}{\mathsf{bd}}
\newcommand{\bdc}{\lambda}
\newcommand{\co}[1]{\overline{#1}}
\newcommand{\rank}{\mathsf{rk}}

\newcommand{\bag}{\textsf{bag}}
\newcommand{\flow}{\textsf{flow}}
\newcommand{\flowp}{\textsf{flow}^*}
\newcommand{\cc}{\texttt{cc}}
\newcommand{\adh}{\mathsf{adh}}
\newcommand{\width}{\mathsf{width}}

\newcommand{\contr}{/}
\newcommand{\hyperg}{\mathcal{H}}


\newcommand{\rescliqs}{\triangleleft}
\newcommand{\orescliqs}{\triangleright}


\newcommand{\ninc}{N^{\mathsf{inc}}}

\newcommand{\inapp}{$\star$}


\newcommand{\children}{\mathsf{children}}
\newcommand{\troot}{\mathsf{root}}
\newcommand{\parent}{\mathsf{parent}}

\newcommand{\vint}{V_{\mathsf{int}}}
\newcommand{\eint}{E_{\mathsf{int}}}


%TODO, define in defs: 

\newcommand{\resgcliqs}{\diamond}





\newcommand{\lmap}{\mathcal{L}}
\newcommand{\leaves}{L}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\torso}{\mathsf{torso}}


\newcommand{\runtime}{\mathsf{RT}}
\newcommand{\oruntime}{\mathsf{ORT}}


%Define in Bodlaender section
\newcommand{\elim}{*}


%Define in superbd editing section
\newcommand{\refiset}{\mathfrak{T}}
\newcommand{\compset}{\mathfrak{C}}

% Define in the section about tangles
\newcommand{\bw}{\mathsf{bw}}
\newcommand{\tw}{\mathsf{tw}}
\newcommand{\wl}{\mathsf{wl}}
\newcommand{\tang}{\mathscr{T}}


% TODO: define
\newcommand{\prop}{\Pi}


% Random
\newcommand{\wilog}{without loss of generality\xspace}


% For lean
\newcommand{\pull}{\mathsf{pull}}
\newcommand{\forget}{\mathsf{forget}}
\newcommand{\paths}{\mathscr{P}}

\newcommand{\ddeg}{\Delta}


\newcommand{\ins}{\mathcal{I}}


\newcommand{\tuukka}[1]{\todo[color=green!40]{Tuukka: #1}}
\newcommand{\tuukkain}[1]{\todo[size=\normalsize,inline,color=green!40]{Tuukka: #1}}

\newcommand{\mikkel}[1]{\todo[color=orange!40]{Mikkel: #1}}
\newcommand{\mikkelin}[1]{\todo[size=\normalsize,inline,color=orange!40]{Mikkel: #1}}
